Closed-form Solution for IMU based LSD-SLAM Point Cloud Conversion into the Scaled 3D World Environment

SLAM is a very popular research stream in computer vision and robotics nowadays. For more effective SLAM implementation it is necessary to have reliable informa- tion about the environment, also the data should be aligned and scaled according to the real world coordinate system. Monocular SLAM research is an attractive sub-stream, because of the low equipment cost, size and weight. In this paper we present a way to build a conversion from LSD-SLAM coordinate space to the real world coordinates using a true metric scale with IMU sensor data implementation. The causes of differences between the real and calculated spaces are explained and the possibility of conversions between the spaces is proved. Additionally, a closed-form solution for inter space trans- formation calculation is presented. The synthetic method of generating high level accurate and well controlled input data for the LSD-SLAM algorithm is presented. Finally, the reconstructed 3D environment representation is delivered as an output of the implemented conversion.

==> AdditonalMeasuring.tex <==
This is to be used for the purpose of path planning,
particularly to scale the measurement obtained with camera to the feature point distance ("Follow Me", for example). 
\hl{Sergey: I don't understand this last sentence.}


% Scene parameters table ******************************************************
\begin{table}[ht]
% title of the table
\caption{SCENE PARAMETERS}  
\centering 										% centering table 
\begin{tabularx}{0.45\textwidth}{X|l}		    % creating eight columns 
\hline\hline 									% inserting double-line   
Path length 						& 				\\ 
\hline
Frames number   					& 	7000 		\\ 
\hline
Linear motion speed					&				\\
\hline\hline
\end{tabularx} 
\label{tab:sceneParams} 
\end{table}  
%********************************************************************************

\begin{figure}[ht]
\centering
  \includegraphics[width=\linewidth]{5MeasuringResults/scaledPath.jpg}
\caption{\hl{Scaled output coordinates}}
\label{fig:scaledPath}
\end{figure}

% Rotation  and translation calculation results
\subsection{Rotation  and translation calculation results}
\hl{Rotate path}

\hl{synchronize frames after end of initialization}

\hl{Analyzing distance between result}

% Results representation and analyzing
\subsection{Results representation and analyzing}

\hl{Build scaled point cloud}

\hl{Analyze distance to STL geometry}

\hl{Represent Octree map}

% RSULTS
As a first attempt to analyze initialization time, the same idea may be used, as it is described in []. 
It is necessary to calculate a \hl{scale factor of vectors - Sergey: I don't understand this} in order to achieve system stabilization. 
The results in Fig.\ref{fig:scaleFactor} show the scaling factors for all the key-frames (blue line). 

After the first 1100 initialization key-frames (marked as red) the scale factor is stable for the rest of the key-frames (marked as black).

\hl{Sergey: This paragraph was a little unclear. Please check carefully what I wrote. Furthermore, I understand that the blue line represent scale factors that you can read off on the left vertical axis. However, what value does the red and black marks represent?}

These scale factors were used in order to scale the LSD-SLAM path. The result is shown in Fig.\ref{fig:scaledPath}. 

Clearly, the two paths (LSD-SLAM and ground truth) are approximately the same scale, however the orientation results need an improvement that would be valuable. The section \ref{sub:problemDefination} describes the expected improvement explanation. 
\hl{Sergey: Do you have any idea why the orientation still is incorrect?} 

% CONCLUSION 

Additional data received from an IMU sensor can be used to estimate SLAM point cloud alignment with a real world coordinate system. 
\hl{The results of the mentioned point cloud alignment can be effectively used by octree algorithm for final reconstruction of the targeted 3D model. 
Sergey: you have not given any octree results yet, therefore I don't think you should say anything about it. 
The contribution of the paper is sufficient and adding an octree afterwards is not very difficult. 
By keeping the octree stuff in the paper, you create the impression for the reader that there is going to be some significant results using octrees.
So, rather take this sentence out.}
Thus, the resulting model can be used for path planning tasks.

In future, it should bring a recognizable benefit to put the conversion matrix to the feedback branch of the system. 
Using IMU (measured orientation and scale factor) as an input for tracking calculation instead of estimated camera position orientation \hl{will reduce initialization time. Sergey: where did you demonstrate this?} 
In this case, the output of the system will be scaled and the axes will be aligned without any additional calculation. 
This approach will fully support real-time solutions and can be used as a distance detector.

\hl{P.S. If there is no IMU implemented, odometry can be used. Fixed camera position expected (for position find).

??? RGB-D have not information about orientation, so need align to.}




% Scene parameters table ******************************************************
\begin{table}[ht]
% title of the table
\caption{SCALED SCENE PARAMETERS}  
\centering 										% centering table 
\begin{tabularx}{0.45\textwidth}{X|l}		    % creating eight columns 
\hline\hline 									% inserting double-line   
Path length 						& 				\\ 
\hline
Frames number   					& 	7000 		\\ 
\hline
Linear motion speed					&				\\
\hline\hline
\end{tabularx} 
\label{tab:sceneParams} 
\end{table}  
%********************************************************************************
